Neural Strands: Learning Hair Geometry and Appearance from Multi-View Images

We present Neural Strands, a novel learning framework for modeling accurate hair geometry and appearance from multi-view image inputs. The learned hair model can be rendered in real-time from any viewpoint with high-fidelity view-dependent effects. Our model achieves intuitive shape and style control unlike volumetric counterparts. To enable these properties, we propose a novel hair representation based on a neural scalp texture that encodes the geometry and appearance of individual strands at each texel location. Furthermore, we introduce a novel neural rendering framework based on rasterization of the learned hair strands. Our neural rendering is strand-accurate and anti-aliased, making the rendering view-consistent and photorealistic. Combining appearance with a multi-view geometric prior, we enable, for the first time, the joint learning of appearance and explicit hair geometry from a multi-view setup. We demonstrate the efficacy of our approach in terms of fidelity and efficiency for various hairstyles.

==> imgs_tex/coarse2fine.tex <==
% \begin{figure}
% \centering
% \begin{tikzpicture}

% \newcommand\Shift{3.2}
% \newcommand\TextY{-2.0}


% \node[inner sep=0pt] at (\Shift*0,0)
%     {\includegraphics[width=.4\columnwidth]{./imgs/coarse2fine/no_coarse2fine.png}};
% % \node[inner sep=0pt] at (\Shift*1,0)
% %     {\includegraphics[width=.32\columnwidth]{./imgs/coarse2fine/no_root2tip.png}};
% \node[inner sep=0pt] at (\Shift*1,0)
%     {\includegraphics[width=.4\columnwidth]{./imgs/coarse2fine/full_system.png}};

% %text at the bottom
% \node at (\Shift*0, \TextY) {\footnotesize No coarse-to-fine};
% % \node at (\Shift*1, \TextY) {\footnotesize w c2f w/o r2t };
% \node at (\Shift*1, \TextY) {\footnotesize With coarse-to-fine};
% % \node at (\Shift*3, \TextY) {\footnotesize G.T.};

% \end{tikzpicture}
% \caption{ \ALEX{Coarse-to-fine} } \label{fig:coarse2fine}
% \end{figure}


\begin{figure}
%\begin{wrapfigure}{R}{0.5\textwidth}
\centering

\captionsetup[subfigure]{font=small,labelfont=small}
%\captionsetup[subfigure]{justification=centering}

\def\haircf{./imgs/coarse2fine/no_coarse2fine.png} %scooter
\newlength{\WCF}
\newlength{\HCF}
\settowidth{\WCF}{\includegraphics{\haircf}}
\settoheight{\HCF}{\includegraphics{\haircf}}



  \subcaptionbox{No coarse-to-fine \\nor root-to-tip\label{fig:a}}%
  {\includegraphics[  trim=.0\WCF{} .15\HCF{} .0\WCF{} .11\HCF{},clip,   width=0.47\linewidth]{./imgs/coarse2fine/no_coarse2fine.png}}
%   \hspace{\fill}
    \hspace{0.0cm}
  \subcaptionbox{With coarse-to-fine \\and root-to-tip\label{fig:b}}%
  {\includegraphics[  trim=.0\WCF{} .15\HCF{} .0\WCF{} .11\HCF{},clip,   width=0.47\linewidth]{./imgs/coarse2fine/full_system.png}}


%   \vspace{-2mm}
  \caption{ Our coarse-to-fine and root-to-tip optimization of the shape texture helps the network converge to the correct shape.  }\label{fig:coarse2fine}
%   \caption{ Coarse-to-fine optimization. Optimizing the shape descriptor for each strand individually can lead the optimization to get stuck in bad local minima. Enabling a coarse-to-fine optimization of the scalp texture and a root-to-tip optimization helps the network converge to the correct shape.  }\label{fig:coarse2fine}
%   \vspace{-5mm}
\end{figure}
%\end{wrapfigure}

==> imgs_tex/hair_transfer.tex <==
\begin{figure}
\centering
\begin{tikzpicture}

\newcommand\Shift{2.0}
\newcommand\TextY{-2.0}


\node[inner sep=0pt] at (\Shift*0,0)
    { \missingfigure{Hair transfer} };



\end{tikzpicture}
\caption{ \ALEX{Hair transfer} } \label{fig:hair_transfer}
\end{figure}

==> imgs_tex/latent_space.tex <==
\begin{figure}
\centering
\begin{tikzpicture}

\newcommand\Shift{2.0}
\newcommand\TextY{-2.0}


\node[inner sep=0pt] at (\Shift*0,0)
    { \missingfigure{Latent space interpolation} };



\end{tikzpicture}
\caption{ \ALEX{Latent space} } \label{fig:latent_space}
\end{figure}

==> imgs_tex/new_hairstyle.tex <==
\begin{figure}
\centering
\begin{tikzpicture}

\newcommand\Shift{2.0}
\newcommand\TextY{-2.0}


\node[inner sep=0pt] at (\Shift*0,0)
    { \missingfigure{New hairstyle} };



\end{tikzpicture}
\caption{ \ALEX{New hairstyles by masking the neural scalp texture} } \label{fig:new_hairstyle}
\end{figure}

==> imgs_tex/no_appearance.tex <==
% \begin{figure}
% \centering
% \begin{tikzpicture}

% \newcommand\Shift{3.5}
% \newcommand\TextY{-2.0}


% \def\noApp{./imgs/no_appearance/noapp_crop.png} %scooter
% \newlength{\WA}
% \newlength{\HA}
% \settowidth{\WA}{\includegraphics{\noApp}}
% \settoheight{\HA}{\includegraphics{\noApp}}



% \node[inner sep=0pt] at (\Shift*0,0)
%     {\includegraphics[ trim=.2\WA{} .1\HA{} .2\WA{} .1\HA{},clip, width=.4\columnwidth]{./imgs/no_appearance/noapp_crop.png}};
% % \node[inner sep=0pt] at (\Shift*1,0)
% %     {\includegraphics[width=.32\columnwidth]{./imgs/coarse2fine/no_root2tip.png}};
% \node[inner sep=0pt] at (\Shift*1,0)
%     {\includegraphics[   trim=.2\WA{} .1\HA{} .2\WA{} .1\HA{},clip, width=.4\columnwidth]{./imgs/no_appearance/app_crop.png}};

% %text at the bottom
% % \node at (\Shift*0, \TextY) {\footnotesize No coarse-to-fine};
% % \node at (\Shift*1, \TextY) {\footnotesize w c2f w/o r2t };
% % \node at (\Shift*1, \TextY) {\footnotesize With coarse-to-fine};
% % \node at (\Shift*3, \TextY) {\footnotesize G.T.};



% \end{tikzpicture}
% \caption{ \ALEX{No appearance  loss vs with appearance loss} } \label{fig:no_app}
% \end{figure}



\begin{figure}[t]
\centering

\def\hairapp{./imgs/no_appearance/noapp_crop.png} %scooter
\newlength{\WAPP}
\newlength{\HAPP}
\settowidth{\WAPP}{\includegraphics{\hairapp}}
\settoheight{\HAPP}{\includegraphics{\hairapp}}



\captionsetup[subfigure]{justification=centering}
  \subcaptionbox{No appearance loss\label{fig:a}}%
  {\includegraphics[  trim=.2\WCF{} .1\HCF{} .2\WCF{} .1\HCF{},clip,   width=0.45\linewidth]{./imgs/no_appearance/noapp_crop.png}}
%   \hspace{\fill}
  \subcaptionbox{With appearance loss\label{fig:b}}%
  {\includegraphics[  trim=.2\WCF{} .1\HCF{} .2\WCF{} .1\HCF{},clip,   width=0.45\linewidth]{./imgs/no_appearance/app_crop.png}}


  \caption{ Joint optimization. Using only the geometry loss, the hair strand can look unrealistic and penetrate through geometry. Using a joint loss of both geometry and appearance helps the strand align better with the line-segments.  }\label{fig:no_app}
\end{figure}

==> imgs_tex/synthetic.tex <==
\begin{figure}[t]
%\begin{wrapfigure}{L}{0.5\textwidth}
	\begin{center}
		\includegraphics[width=0.49\textwidth]{./imgs/synthetic/synthetic01.png}
	\end{center}
% 	\vspace{-6mm}
	\caption{ Synthetic data and geometry reconstructions. From left: GT image, LMVS geometry, our geometry, GT geometry. Note that the strands from LMVS are segmented and not connected to the scalp.} 
	\label{fig:synthetic}
	%\vspace{-4mm}
\end{figure}
%\end{wrapfigure}

==> sections/10conclusion.tex <==
%\vspace{-1mm}
%In this work, we have proposed the first end-to-end learning framework for simultaneously modeling the geometry and appearance of hair from multi-view input, which has not only achieved superior quality compared to other neural rendering methods, but also enabled intuitive editing and control of the hair. 

%However, our approach is still limited when dealing with very complicated hairstyles like the hair-bun in the third row of \reffig{fig:qualitative_compare} where it's challenging to infer the exact topology of the hair since most of it is occluded. Stronger priors for hairstyles learned from various subjects could help alleviate these issues. In spite of a large variety of strand samples to train our strand generator, it may still lack the capacity to represent any hair strand. The stand fitting thus may be prone to local minima, resulting in the estimation to deviate from the captured strands. Incrementally learning the strand generator from the captured data may help. Although our hair model is fully editable, due to the complicated light transport, the generated appearance may not generalize to large hair movement, since lighting effects, like shadows, may be baked in the learned appearance. We will take it as future work to explore more physics-aware rendering since strand-level geometry is available from our model.  


\begingroup
\NEW{
In this work, we have proposed the first joint learning framework for simultaneously modeling the geometry and appearance of hair from multi-view input, which has not only achieved superior quality compared to other neural rendering methods, but also enabled intuitive editing and control of the hair. 
% This opens new doors for AR/VR applications in which the ability to render a human avatar with photorealistic hair in real-time is crucial for social telepresence.
}
\endgroup



==> sections/8applications.tex <==

We show various applications that are now possible with our hair representation by editing the neural scalp texture. 

\subsection{Virtual haircut}
By having an explicit strand, we can trim its length to any desired value and let the neural renderer infer how the hair would look like at the new length. We show that the UNet generalizes and produces realistic appearance even for this hair configuration that was never seen during training~\reffig{fig:hair_manipulation}.
% \input{imgs_tex/grow.tex}

% Since we also have an explicit mesh of the bald head, we can also trim parts of the hair and leaving others at full length, therefore creating a mohawk hairstyle~\reffig{fig:new_hairstyle} This can be easily done by defining a mask on the scalp texture.
% \input{imgs_tex/new_hairstyle.tex}

\subsection{Hair animation}
The explicit hair strands can also be deformed by slightly modifying the direction between adjacent strand nodes to convey a sense of movement of hair blowing in the wind. 
In~\reffig{fig:hair_manipulation} we show examples of animating the hair the appearance inferred for this novel hair configuration. 
More complex methods of animating based on mass-spring systems can also be used but they lie outside of the scope of this article.
% \input{imgs_tex/animation.tex}

\input{imgs_tex/hair_manipulation.tex}


% \subsection{Latent space manipulation}
% Apart from explicitly deforming the strand vertices, we can also directly manipulate the neural scalp texture for the shape of the strands. Since the strand VAE learns a compact latent space for the shape, we identify that some dimensions of the shape $z$ vector, encodes meaningful deformations like curliness, length, etc. We modify the latent representation along these dimensions and we decode new strands. The neural renderer generalizes enough to create realistic appearance for these new strand configurations even if their shape was never seen during training.
% \input{imgs_tex/latent_space.tex}

% \subsection{Hair transfer}
% \todo[inline]{Not sure yet how doable it is and it's currently on my low-priority bucket.}
% \input{imgs_tex/hair_transfer.tex}





==> sections/sections.tex <==
Introduction 
what was not possible before, what is now
Related work 
Method 
        Geometry fitting
        Scalp mesh (talk about flame fitting)
        Strand generator network ( talk about the network inspired by neural ode)
        Strand generator training (use usc, augment it a lot)
        Strand fitting ( optimize a scalp texture, keep the model frozen and use chamfer loss towards line-mvs)
    Appearance fitting
        Neural rendering ( we rasterize feature to screen and neural render them. similar to DNR. use l1+lpips loss) 
        Hair transparency (hair especially is very transparency, we add an alpha loss, by erosion and dilation)
        Compositing (we render also body, background and hair and compose them all together)
    Joint training (talk about joint training of both geoemtry and apperence)
        Differentiable rasterizer (talk about ways of getting the gradients in 2D. We use a softmax splatting operator)
        Coarse2fine optimization (talk about optimizing the scap textures in a coarse-to-fine manner and geometry also in a root-to-tip. Coarse to fine is done by blurring in the backward pass and root-to-tip by masking the gradients in the backward pass)
Results 
    Compare with nerf, NV, MVP qualitatively 
    Compare in terms of psnr, lpips, ssim etc
    Compare completeness of the strands wrt to line-mvs on syntehtic sausalito data 
    Image of novel view synthesis ( an image of the same subject rotated)
    Coarse2fine vs not coarse2fine ( when we don't use coarse to fine, the strands are a mess)
    Comparison with gan-based 
    compare with point rendering vs line rendering
Applications 
    Hair growing (grow the hair from 0,1 or maybe even grow it beyond 1)
    Hair movement (move the strands slightly, hope that the unet doesnt explode)
    Hair transfer (transfer the scalp apperence texture from one person to another)
    Hair editing (edit the latent space of the strands, try to make it curlier for example and hope that the unet renderer doesnt explode)
Limitations 
    Fitting of strands is NP-hard 
    UNet can flicker if the geometry is not good
    Gradients from 2D rasterization can be unstable as mentioned in ADOP, NUPG and other differentiable rasterizers. 

==> tables/quantitative1.tex <==

% \begin{table}
% \begin{center}
% \begin{tabular}{ |c|c|c| } 
% %  \hline
%  NeRF & MVP & Ours \\ 
%  cell4 & cell5 & cell6 \\ 
%  cell7 & cell8 & cell9 \\ 
%  \hline
% \end{tabular}
% \caption{Your caption.} \label{tab:quantitative}
% \end{center}
% \end{table}

% \vspace{-5mm}

\begin{table}[t]
%\begin{wraptable}{R}{0.5\textwidth}
\small
\centering
%  \begin{tabularx}{\columnwidth}{r | c c c }
% \begin{tabular*}{\columnwidth}{r  @{\extracolsep{\fill}}  | c c c }

 \caption{
Quantitative comparison between NeRF, MVP and our approach. 
We perform better under the perceptual metric (LPIPS) indicating that ours have more realistic looking hairs. 
Our method can render a static hair in real-time ($>$25 fps) and dynamic strands at interactive rates ($>$13 fps).
%  Quantitative comparison between NeRF, MVP and our approach. Our method can render in real-time a static hair and at interactive rates if we also perform strand generation at every frame. We perform better under the perceptual metric LPIPS and this leads to more realistic looking hairs. 
 }
\begin{tabular}{r   | c c c }
 & \shortstack{NeRF} & \shortstack{MVP} & \shortstack{Ours} \\
 \hline
 PSNR ($\uparrow$)   &  31.71  &  \textbf{32.82} &  31.30\\
 SSIM ($\uparrow$)   &  0.9383 &  \textbf{0.9599} &  0.9452\\
 LPIPS ($\downarrow$)   &  0.1598 &  0.1226 &  \textbf{0.0811}\\
\hline

 decode (strand gen) ($\downarrow$)   & -  & \textbf{20.40} & 34.54\\
 render ($\downarrow$)   & -  & 81.60 & \textbf{38.82} \\
 total (ms) ($\downarrow$)   & 27,910 &  102.00 &  \textbf{73.36}\\
%  strand gen ($\downarrow$)   & -  & - & 34.54\\
%  render ($\downarrow$)   & -  & - & 38.82 \\
%  total ($\downarrow$)   & 27910.0000 &  102.0 &  \textbf{73.36}\\
 \end{tabular}
 
% \begin{tabular}{c|ccc|c}
%     & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & render $\downarrow$ \\
%     \hline
%     \shortstack{NeRF}   &  31.64  &  0.9383  &  0.1544  &  27,910  \\
%     \shortstack{MVP}    &  \textbf{32.72}  &  \textbf{0.9603}  &  0.1178  &  102.00  \\
%     \shortstack{Ours}   &  30.90  &  0.9363  &  \textbf{0.0837}  &  \textbf{38.82}  \\
% \end{tabular}

 %\vspace{-2mm}

 %\vspace{-2mm}
 \label{tab:quantitative_compare}
\end{table}
%\end{wraptable}





